Recursive Algorithms for Distributed Forests of Octrees

The forest-of-octrees approach to parallel adaptive mesh refinement and coarsening (AMR) has recently been demonstrated in the context of a number of large-scale PDE-based applications. Although linear octrees, which store only leaf octants, have an underlying tree structure by definition, it is not often exploited in previously published mesh-related algorithms. This is because the branches are not explicitly stored, and because the topological relationships in meshes, such as the adjacency between cells, introduce dependencies that do not respect the octree hierarchy. In this work we combine hierarchical and topological relationships between octree branches to design efficient recursive algorithms. We present three important algorithms with recursive implementations. The first is a parallel search for leaves matching any of a set of multiple search criteria. The second is a ghost layer construction algorithm that handles arbitrarily refined octrees that are not covered by previous algorithms, which require a 2:1 condition between neighboring leaves. The third is a universal mesh topology iterator. This iterator visits every cell in a domain partition, as well as every interface (face, edge and corner) between these cells. The iterator calculates the local topological information for every interface that it visits, taking into account the nonconforming interfaces that increase the complexity of describing the local topology. To demonstrate the utility of the topology iterator, we use it to compute the numbering and encoding of higher-order $C^0$ nodal basis functions. We analyze the complexity of the new recursive algorithms theoretically, and assess their performance, both in terms of single-processor efficiency and in terms of parallel scalability, demonstrating good weak and strong scaling up to 458k cores of the JUQUEEN supercomputer.

==> tikzlibraryquadtree.code.tex <==
% This file defines macros for making quadtree diagrams in tikz pictures.
% It depends on the tikz library for trees, so you file must include
%
% \usetikzlibrary{trees}
% \usetikzlibrary{quadtree}

% This puts a quadrant centered at the current location.
\def\quadrant{+(-1cm,-1cm) rectangle +(1cm,1cm) (0,0)}

% Morton order growth function
\tikzstyle{morton order}=[growth function=\quadtree@morton,
                          level distance=\quadtree@sqrt2,
   edge from parent path={(\tikzparentnode.center) (\tikzchildnode.center)}]

% Three options that control the placement of leaves

% Places space between leaves: the space is the same at each level, so this only
% works if the size of the leaves is less than the absolute space
\tikzset{quadtree absolute space/.initial=0.0}
% Places space between leaves proportional to the size of the leaves
\tikzset{quadtree relative space/.initial=0.0}
% Shrinks a leaf towards its center (after applying the above spaces)
\tikzset{quadtree scale/.initial=1.0}

\def\quadtree@morton{%
  \ifnum\tikznumberofcurrentchild=1\relax%
    \c@pgf@counta=-135\relax%
  \else\ifnum\tikznumberofcurrentchild=2\relax%
    \c@pgf@counta=-45\relax%
  \else\ifnum\tikznumberofcurrentchild=3\relax%
    \c@pgf@counta=135\relax%
  \else%
    \c@pgf@counta=45\relax%
  \fi\fi\fi
  \pgftransformscale{.5*(1-2^(\the\tikztreelevel-1)*%
(\pgfkeysvalueof{/tikz/quadtree absolute space})-%
(\pgfkeysvalueof{/tikz/quadtree relative space}))}%
  \pgftransformshift{\pgfpointpolar{\the\c@pgf@counta}%
  {\quadtree@sqrt2 * (2 - (1 -2^(\the\tikztreelevel-1)*%
(\pgfkeysvalueof{/tikz/quadtree absolute space})-%
(\pgfkeysvalueof{/tikz/quadtree relative space})))/%
(1-2^(\the\tikztreelevel-1)*(\pgfkeysvalueof{/tikz/quadtree absolute space})-
(\pgfkeysvalueof{/tikz/quadtree relative space}))}}
  \pgftransformscale{(\pgfkeysvalueof{/tikz/quadtree scale})}
}

\def\quadtree@sqrt2{1.41421356237310 cm}

% Example usage:
%
%  \draw [morton order,quadtree absolute space=0.05] coordinate
%    child {[red]\quadrant}
%    child {[green]\quadrant}
%    child {
%      child {[green]\quadrant}
%      child {
%        child {[green]\quadrant}
%        child {[blue]\quadrant}
%        child {[red]\quadrant}
%        child {[green]\quadrant}}
%      child {
%        child {[green]\quadrant}
%        child {[blue]\quadrant}
%        child {
%          child {[green]\quadrant}
%          child {[blue]\quadrant}
%          child {[red]\quadrant}
%          child {[green]\quadrant}}
%        child {[green]\quadrant}}
%      child {[red]\quadrant}
%      child {[green]\quadrant}}
%    child {[blue]\quadrant};

